An Evasion and Counter-Evasion Study in Malicious Websites Detection

Malicious websites are a major cyber attack vector, and effective detection of them is an important cyber defense task. The main defense paradigm in this regard is that the defender uses some kind of machine learning algorithms to train a detection model, which is then used to classify websites in question. Unlike other settings, the following issue is inherent to the problem of malicious websites detection: the attacker essentially has access to the same data that the defender uses to train its detection models. This 'symmetry' can be exploited by the attacker, at least in principle, to evade the defender's detection models. In this paper, we present a framework for characterizing the evasion and counter-evasion interactions between the attacker and the defender, where the attacker attempts to evade the defender's detection models by taking advantage of this symmetry. Within this framework, we show that an adaptive attacker can make malicious websites evade powerful detection models, but proactive training can be an effective counter-evasion defense mechanism. The framework is geared toward the popular detection model of decision tree, but can be adapted to accommodate other classifiers.

==> realdata.tex <==
\section{Evaluating Effectiveness of the Counter-Evasion Algorithms}
\label{sec:evaluating-framework}

\subsection{Data Description}


%\paragraph*{{\bf Data Description}.}
The dataset used in this paper consists of a 40-day URLs. 
Malicious URLs are downloaded from blacklists: \url{compuweb.com/url-domain-bl.txt}, \url{malware.com.br}, \url{malwaredomainlist.com}, \url{zeustracker.abuse.ch} and \url{spyeyetracker.abuse.ch} and further confirmed with the high-interaction client honeypot Capture-HPC\cite{citeulike:5765320}. Benign URLs are obtained from \url{alexa.com}, which lists the top 10,000 websites that are supposed to be well protected. The test of blacklist URLs using high-interaction client honeypot confirmed our observation that some or many blacklist URLs are not accessible any more and thus should not be counted as malicious URLs.

\ignore{
The dataset for our case study was collected by an automatical script, which will routinely obtained benign and malicious URL list for 40 days period of time, which happened in consecutive days from 02/01/2012 to 03/11/2012. The malicious URLs list are downloaded from blacklists and are confirmed as malicious by the high-interaction client honeypot Capture-HPC version 3.0  \cite{citeulike:5765320}. The malicious URL list are from the following blacklists:
\url{compuweb.com/url-domain-bl.txt}, \url{malware.com.br}, \url{malwaredomainlist.com}, \url{zeustracker.abuse.ch} and \url{spyeyetracker.abuse.ch}. Although the blacklists are updated frequently, some malicious websites have very short life time, which are not accessible or malicious by the time when we tried to access it. Although high-interaction client honeypot has false positive, consider the fact that these malicious URLs are from black list and our experiment is conducted at the same day blacklist URLs are released, so it's safe to say all the malicious URLs of our dataset are actually malicious.
The test of blacklist URLs using high-interaction client honeypot confirmed our observation that some or many blacklist URLs are not accessible any more and thus should not be counted as malicious URLs. The benign URLs are obtained from \url{alexa.com}, which lists the top 10,000 websites that are supposed to be well protected. By eliminating non-accessible benign websites, the average number of benign websites in 40 days are 9501.
}%EOI

%!Table \ref{table:data-description} shows 
The daily average number of malicious websites listed in blacklists is 6763 %!during the 40 days period
 and the daily average number of malicious websites after being verified by Capture-HPC is 838. The total number of distinct malicious websites we found in 40 days are 17091. The daily average number of benign websites is 10,000. By eliminating non-accessible benign websites, the daily average number of benign websites is 9501 in 40 days.
According to \cite{url:oakland:11} and our experiment results, it can achieve best detection rate, when the rate between the number of benign websites and malicious websites are 4:1. So we choose all malicious websites and 4 times of benign websites as our training and testing data.

\ignore{%!
\begin{table}[!hbtp]
\caption{Data summary}
\label{table:data-description}
\centering
{\scriptsize
\begin{tabular}{|c|c|c|c|}
\hline
Website  & Daily Ave.  \# of        & Daily Ave. \# of   & Total \# of Distict \tabularnewline
Category &  Websites  &  Verified Websites  & Websites \tabularnewline
\hline
Benign Websites& 10,000 & 9,501  & 10,000  \tabularnewline
\hline
Malicious Websites& 6,763   & 838     & 17,091  \tabularnewline
\hline
\end{tabular}
}

\end{table}
} %!

\subsection{Effectiveness of the Evasion Attacks}
\label{sec:power-of-adaptive-attack}
%!In order to evaluate the evasion power of adaptive attacks, we evaluate $M_0(D_1)$,
%!where $M_0$ is learned from $D'_0$ and $D_1$ is the output of adaptive attack algorithm ${\sf AA}$.
%run the adaptive attack algorithms to see how the manipulated feature vectors can evade detection.
%!Our experiments are based on a 40-day dataset, where for each day:
%!$D'_0$ consists of 340--722 malicious websites (with mean 571) as well as 2,231--2,243 benign websites (with mean 2,237);
%!$D_0$ consists of 246--310 malicious websites (with mean 282) as well as 1,124--1,131 benign websites (with mean 1,127).
%!As mentioned above, we consider the data-aggregation cross-layer method,
%!while considering single-layer (i.e., application and network) method for comparison purpose.
%In the data-aggregation cross-layer method, application-layer features and network-layer features corresponding to the same URL are simply concatenated together
%to represent the URL in question. Although this method is slightly less effective than
%the XOR-aggregation cross-layer method \cite{codaspy13:li},
%where a website is classified as malicious if (i) both the application-layer classifier and the network-layer classifier say so,
%or (ii) in the case only one of the application-layer and network-layer classifiers says it is malicious,
%the website is analyzed by a backbend dynamic analysis engine.
%The reason is that the XOR-aggregation method will become very complicated when dealing with cross-layer constraints
%(i.e., some application-layer features are correlated to some network-layer features),
%because it treats application-layer and network-layer classifiers separately and can causing cascading side-effect when maintaining constraints.
%In contrast, cross-layer correlations constraints are easy to handle in the data-aggregation method because
%the application- and network-layer features are treated together.

\ignore{
We first highlight some manipulation constraints that are enforced in our experiments.
%implemented in our experiments were  (we do not list all the details because it will become lengthy):
\begin{itemize}
\item{\bf Domain constraints}:
The length of URLs ({\tt URL\_length}) cannot be arbitrarily manipulated because it must include hostname, protocol name,
domain name and directories.
Similarly, the length of webpage content ({\tt Content\_length}) cannot be arbitrarily short.
% host essential parts of HTML page and no less than the sum of script length, http head length and so on.
%The volume of website-to-crawler communications ({\tt App\_bytes}) must be greater than the volume of each website-to-crawler communication.
%The application-layer content length ({\tt app\_bytes}) must be greater than the sum of the lengthes of the crawler-to-server
%({\tt src\_app\_bytes}) and the server-to-crawler ({\tt dst\_app\_bytes}) application-layer contents.
%, which are two different sub-type of {\tt app\_bytes}.

%{\tt app\_packets}: it's value must be greater than the sum of sending application-layer bytes {\tt src\_app\_packets} and receiving application-layer bytes{\tt dst\_app\_packets}.

\item{\bf Correlation constraints}:
%we identified 10 groups of features that are strongly correlated to each other. Features inside group have strong correlation, but there are no overlap among groups.
There are four groups of application-layer features that are strongly correlated to each other;
there are three groups of network-layer features that are strongly correlated to each other;
there are three groups of features that formulate cross-layer constraints.
One group of cross-layer correlation is: the application-layer website content length ({\tt \#Content\_length})
and the network-layer duration time ({\tt Duration}). This is because the bigger the content, the longer the fetching time.
Another group of cross-layer correlations is: the application-layer number of redirects ({\tt \#Redirect}),
the network-layer number of DNS queries ({\tt \#DNS\_query}),
the network-layer number of DNS answers ({\tt \#DNS\_answer}).
This is because more redirects leads to more DNS queries and more DNS answers.

\item{\bf Semantics constraints}:
Assuming the Whois system is not compromised, the following features cannot be manipulated:
website registration date ({\tt RegDate}),
website registration state/province ({\tt Stateprov}),
website registration postal code ({\tt Postalcode}), and
website registration country ({\tt Country}).
%{\tt Updated} (whois updated date).
% may be changed, but can only be change late by previous date.
For malicious websites that use some scripts to launch the drive-by-download attack,
the number of scripts contained in the webpage contents ({\tt \#Scripts}) cannot be 0.
The application-layer protocol feature ({\tt Protocol}) may not be arbitrarily changed (e.g., from ftp to http).
\end{itemize}

} %end of ignore.
Table \ref{table:attack-power} summarizes the results of adaptive attack ${\sf AA}(``J48",M_0,$ $D_0,{\sf ST},{\sf C},{\sf F},\alpha=1)$
based on the 40-day dataset mentioned above. %!, where ${\sf C}$ accommodates the constraints mentioned above.
The experiment can be more succinctly represented as $M_0(D_1)$, meaning that the defender is static (or non-proactive) and
the attacker is adaptive with $\alpha=1$, where $D_1$ is the manipulated version of $D_0$.
Note that in the case of $\alpha=1$, the three adaptation strategies lead to the same $D_1$ as shown in Figure \ref{fig:attack-adaptation-methodologies}.
From Table \ref{table:attack-power}, we find that both manipulation algorithms can effectively evade detection
by manipulating on average 4.31-7.23 features while achieving false-negative rate 87.6\%-94.7\% for ${\sf F}_1$,
and by manipulating on average 4.01-6.19 features while achieving false-negative rate 89.1\%-95.3\% for ${\sf F}_2$
\begin{table}[!htbp]
\caption{Experiment results with $M_0(D_1)$
%, or more precisely ${\sf AA}(``J48",M_0,D_0,{\sf ST},{\sf C},{\sf F},\alpha=1)$,
in terms of average false-negative rate (FN),
average number of manipulated features (\#MF), average percentage of failed attempts (FA).
%, where ${\sf F}\in \{{\sf F}_1, {\sf F}_2\}$.
% (i.e., {\tt parallel-adaptation}, {\tt sequential-adaptation} and {\tt full-adaptation}).
%!where ``average" is over the 40 days of the dataset.%! mentioned above.
%Note that in the case of $\alpha=1$, there is no difference between the three adaptation strategies.
\label{table:attack-power}
}
\centering
{\scriptsize
\begin{tabular}{|l|r|r|r|r|r|r|}
\hline
    & \multicolumn{3}{c|}{${\sf F_1}$} & \multicolumn{3}{c|}{${\sf F_2}$} \\
\hline
  Detection Scheme &  FN & \#MF &FA &  FN & \#MF & FA \\
\hline
J48 Decision Tree&   87.6\% & 7.23 & 12.6\%  & 89.1\% & 6.19& 11.0\%\\
\hline
\end{tabular}
}
\vspace{-0.1in}
\end{table}
%!For the three J48 classifiers based on different kinds of $D_0$ (i.e., network-layer data alone, application-layer data alone and cross-layer data-aggregation),
, which almost always slightly outperforms ${\sf F}_1$.
%! in terms of false-negative rate (FN),
%!average number of manipulated features (\#MF), and average percentage of failed attempts at manipulating feature vectors (FA).
%!Second, data-aggregation cross-layer classifiers are more resilient against adaptive attacks
%!than network-layer classifiers  as well as application-layer classifiers.
%As mentioned above, on average by manipulating 4-7 features, malicious websites can successfully evade from detection system.
%But we may also want to know which exactly features led to evasion? In order to gain some insight into the effect of manipulation, we consider application-layer and network-layer.
%!\vspace{-0.1in}
Having observed the phenomenon that manipulation of some features' values can essentially make the detection schemes useless,
it would be natural to ask {\bf{\em which features are often manipulated for evasion?}} 
To look into the question, we notice that many features are manipulated over the 40 days, but only a few are manipulated often.
%Figure \ref{fig:appmanipulate} summarizes the application-layer features that are manipulated to bypass classifier $M_{0}$.
\ignore{
For application-layer alone, ${\sf F}_1$ most often (i.e., $>150$ times each day for over the 40 days) manipulates the following five application-layer features:
URL length ({\tt URL\_length}), number of scripts contained in website content ({\tt \#Script}),
webpage length ({\tt Content\_length}), number of URLs embedded into the website contents ({\tt \#Embedded\_URL}),
and number of Iframes contained in the webpage content ({\tt \#Iframe}).
In contrast, ${\sf F}_2$ most often (i.e., $>150$ times) manipulates the following three application-layer features:
number of special characters contained in URL ({\tt \#Special\_character}),
number of long strings ({\tt \#Long\_strings}) and
webpage content length
({\tt Content\_length}).
That is, {\tt Content\_length} is the only feature that is most often manipulated by both algorithms.

For network-layer alone, ${\sf F}_1$ most often (i.e., $>150$ times) manipulates the following three features:
% frequently and ${\sf F}_2$ manipulated one single feature frequently, both for more than 150 times (on average of the 40 days).
%The three features ${\sf F}_1$ manipulated are:
number of remote IP addresses ({\tt \#Dist\_remote\_IP}),
duration time ({\tt Duration}), and number of application packets ({\tt \#Local\_app\_packet}).
Whereas, ${\sf F}_2$ most often (i.e., $>150$ times) manipulates the distinct number of TCP ports used by the remote servers ({\tt \#Dist\_remote\_TCP\_port}).
In other words, no single feature is often manipulated by both algorithm.
}

%!Specific to data-aggregation cross-layer detection, 
${\sf F}_1$ most often (i.e., $>150$ times each day for over the 40 days) manipulates
three application-layer features ---  {\tt URL\_length}, {\tt Content\_length}ß,
{\tt \#Embedded\_URLs} ---
and two network-layer features --- {\tt Duration} and  
{\tt \#Local\_app\_packet}.
On the other hand, ${\sf F}_2$ most often (i.e., $>150$ times) manipulates
%We observe the following three features are most frequently (i.e., $>150$ times) manipulated by $F2$:
two application-layer features ---  {\tt \#Special\_characters}
and {\tt Content\_length} --- and one network-layer feature --- {\tt Duration}.
%!Therefore,  {\tt Content\_length} and {\tt Duration} are  most often manipulated by both algorithms.

The above discrepancy between the frequencies that features are manipulated
%phenomenon that some features are manipulated more often than others
can be attributed to the design of the manipulation algorithms.
Specifically, ${\sf F}_1$ seeks to manipulate features that are associated to nodes that are close to the leaves.
In contrast, ${\sf F}_2$ emphasizes on the mismatches between a malicious feature vector and an entire benign path,
which represents a kind of global search and also explains why ${\sf F}_2$ manipulates fewer features.

\ignore{
To answer the second question raised above, it would be ideal if we can directly answer this question by looking into the most-often
manipulated features. Unfortunately, this is a difficult problem because J48 classifiers (or most, if not all, detection schemes based on machine learning),
are learned in a {\em black-box} (rather than {\em white-box}) fashion. 
}


We also want to know {\bf{\em why these features have such high security/evasion significance?}} The issue is important because identifying the ``important" features could lead to deeper insights. We compare the manipulated features to the features that would be selected by a feature selection algorithm for the purpose of training classifiers. To be specific, we use the {\sf InfoGain} feature selection algorithm
because it ranks the contributions of individual features \cite{codaspy13:li}.
We find that among the manipulated features, {\tt URL\_length} is the only feature among the five {\sf InfoGain}-selected application-layer features,
and {\tt \#Dist\_remote\_TCP\_port} is the only feature among the four {\sf InfoGain}-selected network-layer features. This suggests that the feature selection algorithm does not necessarily offer good insights into
the importance of features from a security perspective.

The standard feature-selection algorithms are almost useless to find indicative features from the perspective 
of evading classifiers. There is still gap between our results and the ``optimal" solutions based on security semantics; 
it's an open problem to bridge the gap, because classifiers are ``black-box" that don't really accommodate 
``security semantics" of features. %This problem is left for future investigation.


\ignore{ ???
\begin{table}[!htbp]
\centering
{\scriptsize
\begin{tabular}{|l|r|r|r|r|r|r|}
\hline
    & \multicolumn{3}{c|}{${\sf F_1}$} & \multicolumn{3}{c|}{${\sf F_2}$} \\
\hline
   &  FN & \#MF &FA &  FN & \#MF & FA \\
\hline
network-layer & 93.1\% & 4.29 & 7.5\% &  95.3\% & 4.07 & 5.1\% \\
\hline
application-layer & 91.3\% & 6.00& 9.2\% & 93.3\% & 5.28 & 7.1\% \\
\hline
data-aggregation&  87.4\% & 7.22 & 12.7\%  & 89.1\% & 6.23 & 11.0\%\\
\hline
\end{tabular}
\caption{Experiment results of $M_0(D_1)$ by treating as non-manipulatable the {\sf InfoGain}-selected five application-layer
features and four network-layer features.
Metrics are as in Table \ref{table:attack-power}.
% except that the selected features (five application-layer
%features and four network-layer features) mentioned above are forced not to be manipulated.
%in terms of false-negative rate (FN), number of manipulated features (\#MF), percentage of failed instances (FA), where
%${\sf F}\in \{{\sf F}_1, {\sf F}_2\}$.
%The results are based on the average over 40 days, where for each day $D_0$ is composed of 146--310 malicious websites (with mean 202),
%for each day $D'_0$ is composed of 340--722 malicious websites (with mean 471), and 2231--2243 benign websites (with mean 2237).
%Note that in the case of $\alpha=1$, there is no difference between the three adaptation strategies.
\label{table:attack-power-feature-slection}
}}
\end{table}

%Having identified the features that are often manipulated,
%the next natural question is: {\bf Why them? Or: Are they some kind of ``important" features?}
To answer the second question raised above, it would be ideal if we can directly answer this question by looking into the most-often
manipulated features. Unfortunately, this is a difficult problem because J48 classifiers (or most, if not all, detection schemes based on machine learning),
are learned in a {\em black-box} (rather than {\em white-box}) fashion.  As an alternative, we compare the manipulated features to the features
that would be selected by a feature selection algorithm for the purpose of training classifiers.



To be specific, we use the {\sf InfoGain} feature selection algorithm
%because it was also used in \cite{codaspy13:li} and
because it ranks the contributions of individual features \cite{codaspy13:li}.
We find that among the manipulated features, {\tt URL\_length} is the only feature among the five {\sf InfoGain}-selected application-layer features,
and {\tt \#Dist\_remote\_TCP\_port}
%(the number of distinct TCP ports the webserver used during the conversation with the crawler,
%which can be multiple when the crawler tracks redirects)
is the only feature among the four {\sf InfoGain}-selected network-layer features.
This suggests that the feature selection algorithm does not necessarily offer good insights into
the importance of features from a security perspective. To confirm this, we further conduct the following
experiment by additionally treating {\sf InfoGain}-selected tops features as semantics constraints in {\sf C} (i.e., they cannot be manipulated).
%and by re-running the adaptive attack algorithm ${\sf AA}(``J48",M_0,D_0,{\sf ST},{\sf C},{\sf F},\alpha=1)$.
Table \ref{table:attack-power-feature-slection} (counterparting Table \ref{table:attack-power}) summarizes the new experiment results.
By comparing the two tables, we observe that there is no significant difference between them,
especially for manipulation algorithm ${\sf F}_2$.
This means that {\sf InfoGain}-selected features have little security significance.
%are not fundamental
%to the attack semantics.
%This also hints that it is difficult to defeat adaptive attacks by restricting {\sf InfoGain}-selected features as non-manipulatable.
To sum up, the issue is important because identifying the "important" features could lead to deeper insights.
We find that standard feature-selection algorithms are almost useless for this purpose, and our algorithms can
find more indicative features from the perspective of evading classifiers. There is still gap between our results
and the "optimal" solutions based on security semantics; it is an open problem to bridge the gap because classifiers are
``black-box" models that don't really accommodate "security semantics" of features.




\begin{table}[!htbp]
\centering
{\scriptsize
\begin{tabular}{|l|r|r|r|r|r|r|}
\hline
    & \multicolumn{3}{c|}{${\sf F_1}$} & \multicolumn{3}{c|}{${\sf F_2}$} \\
\hline
   &  FN & \#MF &FA &  FN & \#MF & FA \\
\hline
network-layer     & 62.1\% & 5.88 & 41.6\%  & 80.3\% & 5.07 & 21.6\% \\
\hline
application-layer & 68.3\% & 8.03 & 33.7\%  & 81.1\% & 6.08 & 20.1\% \\
\hline
data-aggregation  & 59.4\% & 11.13 & 41.0\% & 78.7\% & 7.83 & 21.5\%\\
\hline
\end{tabular}
\caption{Experiment results of $M_0(D_1)$ by treating the features that were manipulated by adaptive attack {\sf AA} as non-manipulatable.
Notations are as in Tables \ref{table:attack-power}-\ref{table:attack-power-feature-slection}.
% except the eight manipulated features (five application-layer features and three network-layer features) mentioned in the text are forced not to be manipulated.
\label{table:attack-power-manipulation-slection}
}}
\end{table}


In order to know whether or not the adaptive attack algorithm {\sf AA} actually manipulated some ``important" features,
we conduct an experiments by setting the most-often manipulated features as non-manipulatable.
The features that are originally identified by ${\sf F}_1$ and then set as non-manipulatable are: webpage length ({\tt content\_length}),
number of URLs that are embedded into the website contents ({\tt \#Embedded\_URLs}), number of redirects ({\tt \#Redirect}),
number of distinct TCP ports that are used by the remote webservers ({\tt Dist\_remote\_tcp\_port}), and number of application-layer packets ({\tt Local\_app\_packets}).
Table \ref{table:attack-power-manipulation-slection} summarizes the results.
When compared with Tables \ref{table:attack-power}-\ref{table:attack-power-feature-slection},
we see that the false-negative rate caused by adaptive attacks drops substantially: from about 90\% down to about 60\%
for manipulation algorithm ${\sf F}_1$, and from about 90\% down to about 80\% for manipulation algorithm ${\sf F}_2$.
This means perhaps that the features that are originally identified by ${\sf F}_1$ are more indicative of malicious websites
than the features that are originally identified by ${\sf F}_2$.
Moreover, we note that no feature is manipulated more than 150 times and only two features --- {\tt \#Iframe} (the number of iframes)
and {\tt \#DNS\_query} (the number of DNS query) --- are manipulated more than 120 times by ${\sf F}_1$ and
one feature --- {\tt \#JS\_function} (the number of JavaScript functions) --- is manipulated more than 120 times by ${\sf F}_2$.


} %end of ignore




\subsection{Effectiveness of the Counter-Evasion Algorithms}
\begin{table*}[thb]
\centering
\caption{Cross-layer proactive detection with ${\sf ST}_A={\sf ST}_D$.
For baseline case $M_0(D_0)$, ACC = 99.68\%, true-positive rate TP =99.21\%,
false-negative rate FN=0.79\%, and false-positive rate FP=0.14\%.
%!The primary findings are: the defender can always use proactive detection without worrying about the side-effects (e.g., when the attacker is not adaptive);
%!if the attacker's strategy is {\tt sequential} adaptation, then the defender should {\em not} use the {\tt sequential} strategy.
\label{table:cross-and-aggregation}
{\scriptsize
\begin{tabular}{|l|l|rrrr|rrrr|rrrr|}
\hline
\multirow{2}{*}{Strategy} & \multirow{2}{*}{Manipulation algorithm}  & \multicolumn{4}{c|}{ $M_{0\text{-}8}(D_0)$ }  & \multicolumn{4}{c|}{$M_{0\text{-}8}(D_1)$} &\multicolumn{4}{c|}{$M_{0\text{-}8}(D_9)$ }\\
\cline{3-14}
                        &  &ACC & TP & FN & FP          &ACC & TP & FN & FP        &ACC  & TP & FN & FP \\
\hline
\multirow{3}{*}{${\sf ST}_A={\sf ST}_D$} & ${\sf F}_D={\sf F}_1$ vs. ${\sf F}_A={\sf F}_1$   & 99.59& 99.71  & 0.29  & 0.39 & 95.58 & 92.03 & 7.97 & 3.62   & 95.39 & 92.00  & 8.00   & 3.83 \\ \cline{2-14}
\multirow{4}{*}{$={\tt parallel}$}  & ${\sf F}_D={\sf F}_1$ vs. ${\sf F}_A={\sf F}_2$  																										& 99.27& 99.77  & 0.23  & 0.77 & 78.51 & 25.50 & 74.50 & 9.88  & 78.11 & 32.18  & 67.82  & 11.48    \\ \cline{2-14}
          & ${\sf F}_D={\sf F}_2$ vs. ${\sf F}_A={\sf F}_1$  																								& 99.16& 99.76  & 0.24  & 0.93 & 76.33 & 19.32 & 80.68 & 11.17 & 78.96 & 39.77  & 60.23  & 12.14          \\ \cline{2-14}
 		  & ${\sf F}_D={\sf F}_2$ vs. ${\sf F}_A={\sf F}_2$  																										& 99.59& 99.62  & 0.38  & 0.39 & 93.66 & 90.25 & 9.75 & 5.59   & 96.17 & 92.77  & 7.23   & 3.08          \\ \hline
\multirow{3}{*}{${\sf ST}_A={\sf ST}_D$} & ${\sf F}_D={\sf F}_1$ vs. ${\sf F}_A={\sf F}_1$ & 99.52& 99.69  & 0.31  & 0.45 & 93.44 & 77.48 & 22.52 & 3.05  & 92.04 & 59.33  & 30.67  & 2.99 \\ \cline{2-14}
\multirow{4}{*}{$={\tt sequential}$}  & ${\sf F}_D={\sf F}_1$ vs. ${\sf F}_A={\sf F}_2$  																										& 99.23& 99.70  & 0.30  & 0.82 & 74.24 & 20.88 & 79.22 & 14.06 & 79.43 & 30.03  & 69.97  & 9.38          \\ \cline{2-14}
          & ${\sf F}_D={\sf F}_2$ vs. ${\sf F}_A={\sf F}_1$  																								& 99.27& 99.67  & 0.33  & 0.80 & 77.14 & 29.03 & 70.97 & 12.33 & 82.72 & 40.93  & 59.07  & 7.83          \\ \cline{2-14}
 		  & ${\sf F}_D={\sf F}_2$ vs. ${\sf F}_A={\sf F}_2$   																									& 99.52& 99.53  & 0.47  & 0.50 & 93.44 & 78.70 & 21.30 & 2.10  & 92.04 & 62.30  & 37.70  & 2.11       	\\ \hline
\multirow{3}{*}{${\sf ST}_A={\sf ST}_D$}& ${\sf F}_D={\sf F}_1$ vs. ${\sf F}_A={\sf F}_1$				& 99.68& 99.44 & 0.56  & 0.20  & 96.92 & 96.32 & 3.68  & 2.89  & 95.73 & 92.03 & 7.97 	  & 3.27 \\ \cline{2-14}
\multirow{4}{*}{$={\tt full}$}   & ${\sf F}_D={\sf F}_1$ vs. ${\sf F}_A={\sf F}_2$  																									  & 99.27& 99.58  & 0.42  & 0.72 & 85.68 & 40.32 & 59.68 & 4.38  & 78.11 & 29.99  & 70.01  & 11.00          \\ \cline{2-14}
          & ${\sf F}_D={\sf F}_2$ vs. ${\sf F}_A={\sf F}_1$  																							  & 99.60& 99.66  & 0.34  & 0.40 & 85.65 & 51.84 & 48.16 & 6.93  & 87.61 & 72.99  & 27.01  & 9.01          \\ \cline{2-14}
 		  & ${\sf F}_D={\sf F}_2$ vs. ${\sf F}_A={\sf F}_2$   																									& 99.68& 99.60 &  0.40  & 0.28 & 96.92 & 95.60 & 4.40 & 2.88	 & 95.73 & 90.09  & 9.91   &  2.83		\\ \hline
\end{tabular}
}
}
\vspace{-0.1in}
\end{table*}
\begin{table*}[!htbp]
 \centering
\caption{Proactive detection against adaptive attacks with ${\sf F}_D={\sf F}_A$.
For the baseline case $M_0(D_0)$, we have ACC = 99.68\%, TP =99.21\%, FN=0.79\%, FP=0.14\%.
%!The primary finding is that the {\em full} adaptation strategy may be close to the equilibrium strategy.
\label{table:better-strategies}
{\scriptsize
%\subtable[Manipulation algorithm ${\sf F}_D={\sf F}_A={\sf F}_1$\label{table:F1-resilience}]{
\begin{tabular}{|l|l|rrrr|rrrr|rrrr|}
\hline
\multirow{2}{*}{${\sf ST}_D$ vs. ${\sf ST}_A$} & \multirow{2}{*}{$M_{0\text{-}\gamma}(D_\alpha)$} & \multicolumn{4}{c|}{${\sf ST}_A={\tt parallel}$} & \multicolumn{4}{c|}{${\sf ST}_A={\tt sequential}$}  & \multicolumn{4}{c|}{${\sf ST}_A={\tt full}$} \\
\cline{3-14}
                      &           & ACC & TP & FN & FP & ACC  & TP & FN & FP  & ACC & TP & FN & FP  \\
\hline \hline
\multicolumn{14}{|c|}{Manipulation algorithm ${\sf F}_D={\sf F}_A={\sf F}_1$} \\
\hline
\multirow{2}{*}{${\sf ST}_D={\tt parallel}$}&
%$M_{0\text{-}8}(D_0)$   & 99.59& 99.71 & 0.29 & 0.39     & 99.63& 99.50 & 0.50 & 0.31     & 99.61   & 99.66 & 0.34 & 0.38         \\ \cline{2-14}
% &
$M_{0\text{-}8}(D_1)$                         & 95.58& 92.03 & 7.97 & 3.62     & 94.25& 90.89 & 9.11 &  4.96    & 94.91   & 92.08 & 7.92 & 4.32        \\ \cline{2-14}
 &$M_{0\text{-}8}(D_9)$                           & 95.39& 92.00 & 8.00 & 3.83     & 92.38& 80.03 & 19.97 & 4.89    & 93.19   & 84.32 & 15.68 & 4.54        \\ \hline
\multirow{2}{*}{${\sf ST}_D={\tt sequential}$} &
%$M_{0\text{-}8}(D_0)$& 99.59& 99.77 & 0.23  & 0.37    & 99.52& 99.69 & 0.31 &  0.45    & 99.46   & 99.38 & 0.62 & 0.48         \\ \cline{2-14}
% &
$M_{0\text{-}8}(D_1)$ 	                        & 92.15& 74.22 & 25.78 & 3.93    & 93.44& 77.48 & 22.52 & 3.05    & 92.79   & 76.32 & 23.68 & 3.07        \\ \cline{2-14}
 &$M_{0\text{-}8}(D_9)$                              	& 89.20& 58.39 & 41.61 & 4.11    & 92.04& 59.33 & 30.67 & 2.99    & 88.42   & 57.89 & 42.11 & 3.91        \\ \hline
\multirow{2}{*}{${\sf ST}_D={\tt full}$}  &
%$M_{0\text{-}8}(D_0)$     & 99.82& 99.55 & 0.45 & 0.05     & 99.74& 99.44 & 0.56 & 0.16     & 99.68   & 99.44 & 0.56 & 0.20         \\ \cline{2-14}
% &
$M_{0\text{-}8}(D_1)$                             & 96.24& 94.98 & 5.02 & 3.42     & 96.46& 94.99 & 5.01 & 3.15     & 96.92   & 96.32 & 3.68 & 2.89         \\ \cline{2-14}
 &$M_{0\text{-}8}(D_9)$                              & 94.73& 90.01 & 9.99 & 4.21     & 94.70& 90.03 & 9.97 & 4.23     & 95.73   & 92.03 & 7.97 & 3.27         \\  \hline
%\end{tabular}
%}
%\subtable[Manipulation algorithm ${\sf F}_D={\sf F}_A={\sf F}_2$\label{table:F1-resilience}]{
%\begin{tabular}{|l|l|rrrr|rrrr|rrrr|}
%\hline
%\multirow{2}{*}{${\sf ST}_D$ vs. ${\sf ST}_A$} & \multirow{2}{*}{$M_{0\text{-}\gamma}(D_\alpha)$} & \multicolumn{4}{c|}{${\sf ST}_A={\tt Parallel}$} & \multicolumn{4}{c|}{${\sf ST}_A={\tt Sequential}$}  & \multicolumn{4}{c|}{${\sf ST}_A={\tt Full}$} \\ \cline{3-14}
%                     &             & ACC & TP & FN & FP & ACC & TP & FN & FP & ACC  & TP & FN & FP  \\
\hline
\multicolumn{14}{|c|}{Manipulation algorithm ${\sf F}_D={\sf F}_A={\sf F}_2$} \\
\hline
\multirow{2}{*}{${\sf ST}_D={\tt parallel}$}&
%$M_{0\text{-}8}(D_0)$  & 99.59	& 99.62 & 0.38 & 0.39    & 99.63 & 99.51 & 0.49 & 0.48      & 99.61  & 99.60 & 0.40 & 0.88      \\ \cline{2-14}
% &
$M_{0\text{-}8}(D_1)$                                      	& 93.66	& 90.25 & 9.75 & 5.59    & 94.25 & 88.91 & 11.09 &  3.98    & 94.91  & 89.77 & 10.23 & 3.53            \\ \cline{2-14}
 &$M_{0\text{-}8}(D_9)$                                         & 96.17	& 92.77 & 7.23 & 3.08    & 92.38 & 77.89 & 22.11 & 4.32     & 93.19  & 81.32 & 18.68 & 3.38                 \\ \hline
\multirow{2}{*}{${\sf ST}_A={\tt sequential}$} &
%$M_{0\text{-}8}(D_0)$ 	& 99.19  & 99.50 & 0.50  & 0.83  & 99.52  & 99.53 & 0.47 &  0.50    & 99.46   & 99.70 & 0.30 & 0.49      \\ \cline{2-14}
% &
$M_{0\text{-}8}(D_1)$ 	       	& 90.86	& 70.98 & 29.02 & 4.82   & 93.44 & 78.70 & 21.30 & 2.10     & 92.79  & 72.32 & 27.68 & 4.02                     \\ \cline{2-14}
 &$M_{0\text{-}8}(D_9)$                                         & 88.43	& 53.32 & 46.68 & 3.97   & 92.04 & 62.30 & 37.70 & 2.11     & 88.42  & 57.88 & 42.12 & 3.17            \\ \hline
\multirow{2}{*}{${\sf ST}_A={\tt full}$}  &
%$M_{0\text{-}8}(D_0)$  & 99.63  & 99.59 & 0.41 & 0.34   & 99.74  & 99.60 & 0.40 & 0.33     & 99.68   & 99.60 & 0.40 & 0.28         \\ \cline{2-14}
% &
$M_{0\text{-}8}(D_1)$                         & 95.69	& 93.89 & 6.11 & 3.88    & 96.46 & 94.98 & 5.02 & 3.03      & 96.92  & 95.60 & 4.40 & 2.88             \\         \cline{2-14}
 &$M_{0\text{-}8}(D_9)$                               & 96.06	& 91.46 & 8.54 & 2.89    & 94.70 & 90.99 & 9.01 & 2.32      & 95.73  & 90.09 & 9.91 & 2.83           \\  \hline
\end{tabular}
%}
}
}
\vspace{-0.1in}
\end{table*}
%!The evaluation is based on the metrics defined in Section \ref{sec:data-collection}, namely
%!detection accuracy (ACC), trust-positive (TP), false-negative (FN), and false-positive (FP).
%Note that TP=1-FN, but we still list both for easing the discussion.
%!When the other parameters are clear from the context,
%!we use $M_{0\text{-}\gamma}(D_\alpha)$ to stand for
%!${\sf Eva}({\sf MLA}, M_0, D_0^\dag,{D}_0, {\sf ST}_A, {\sf F}_A,{\sf ST}_D,{\sf F}_D,{\sf C},\alpha,\gamma)$.

%!More specifically, %!the data for proactive training, namely $D_0^\dag$, consists of 333--719 malicious websites (with mean 575) and 2,236--2,241 benign websites (with mean 2,238).
%!For the baseline case of non-proactive detection against non-adaptive attack, namely $M_0(D_0)$, we have average
%!ACC = 99.68\% (detection accuracy), TP =99.21\% (true-positive rate),
%!FN=0.79\% (false-negative rate) and FP=0.14\% (false-positive rate),
%!where ``average" is over the 40 days corresponding to the dataset.
%!This baseline result also confirms the conclusion in  \cite{codaspy13:li}, namely that
%!data-aggregation cross-layer detection can be used in practice, and justifies why we use it in this paper.

Table \ref{table:cross-and-aggregation} summarizes the effectiveness
of proactive defense against adaptive attacks.
We make the following observations.
First, if the defender is proactive (i.e., $\gamma>0$) but the attacker is non-adaptive (i.e., $\alpha=0$),
the false-negative rate drops from 0.79\% in the baseline case
% (i.e., $\alpha=\gamma=0$ or $M_0(D_0)$)
to some number belonging to interval $[0.23\%,0.56\%]$.
% among the combinations of attack strategy ({\sf ST}) and manipulation algorithm ({\sf F}).
The price is: the detection accuracy drops from 99.68\% in the baseline case to some number belonging to interval $[99.23\%,99.68\%]$
%(except the case of ${\sf ST}_A={\sf ST}_D={\tt Parallel}$ and ${\sf F}_D={\sf F}_2$ vs. ${\sf F}_A={\sf F}_1$),
the false-positive rate increases from 0.14\% in the baseline case to some number belonging to interval $[0.20\%,0.93\%]$,
%!and the proactive detection algorithm {\sf PD}'s running time is now $(\gamma+1)$
%!times of the baseline case because of running $M_0(D_\alpha),M_1^\dag(D_\alpha),\ldots,M_\gamma^\dag(D_\alpha)$,
%!which takes on average $0.54(\gamma+1)$ milliseconds to process a feature vector.
%!Note that the running time of the proactive training algorithm {\sf PT} is also $(\gamma+1)$ times of the baseline training algorithm.
%!This can be reasonably ignored because the defender only runs the training algorithms once a day.
The above observations suggest: {\bf the defender can always use proactive detection without worrying about
side-effects (e.g., when the attacker is not adaptive)}. This is because the proactive detection algorithm {\sf PD}
uses $M_0(D_0)$ as the first line of detection.
\begin{figure*}[!hbtp]
\centering
\subfigure[Fixed defender adaptation strategy against varying attacker adaptation strategies,
where both the attacker and the defender use manipulation algorithm ${\sf F}_1$.
We observe that the {\tt FULL} adaptation strategy leads to relatively better detection accuracy.\label{fig:gamma-alpha-f1}]{
\includegraphics[width=0.3\textwidth]{paracc.eps}
\includegraphics[width=0.3\textwidth]{seqacc.eps}
\includegraphics[width=0.3\textwidth]{fullacc.eps}
%\caption{Impact of $\alpha - \gamma$ in the case of ${\sf F}_D={\sf F}_A={\sf F}_1$ under various ``${\sf ST}_D$ vs. ${\sf ST}_A$" combinations.
%\label{fig:gamma-alpha-f1-acc}
}
%\end{figure*}
%
%\begin{figure*}[!hbtp]
%\centering
\subfigure[Fixed defender adaptation strategy against varying attacker adaptation strategies,
where both the attacker and the defender use manipulation algorithm ${\sf F}_2$.
We observe that the {\tt FULL} adaptation strategy leads to relatively better detection accuracy.\label{fig:gamma-alpha-f2}]{
\includegraphics[width=0.3\textwidth]{par2acc.eps}
\includegraphics[width=0.3\textwidth]{seq2acc.eps}
\includegraphics[width=0.3\textwidth]{full2acc.eps}}
\caption{Impact of defender's proactiveness $\gamma$ vs. attacker's adaptiveness $\alpha$ on detection accuracy (average over the 40 days)
under various ``${\sf ST}_D\times {\sf ST}_A$'' combinations,
where $\alpha \in [0,8]$, $\gamma \in [0,9]$, ${\tt PAR}$, ${\tt SEQ}$ and ${\tt FULL}$ respectively stand for ${\tt parallel}$,
${\tt sequential}$ and ${\tt full}$ adaptation strategy, ``${\tt SEQ}$ vs. ${\tt APR}$" means ${\sf ST}_D={\tt sequential}$ and ${\sf ST}_A={\tt parallel}$ etc.
Note that $\gamma-\alpha=a$ is averaged over all possible combinations of $(\alpha,\gamma)$ as long as $\alpha \in [0,8]$ and $\gamma \in [0,9]$,
and that the detection accuracy is averaged over the 40 days. We observe that the detection accuracy in most cases there is a significant increase
in detection accuracy when the defender's proactiveness matches the attacker's adaptiveness.
\label{fig:gamma-alpha-f1-f2}}
\end{figure*}

Second, when ${\sf ST}_A={\sf ST}_D\neq0$,
%the attacker and defender use the same adaptation strategy {\sf ST}
%!(meaning $\alpha>0$ and $\gamma>0$),
it has a significant impact whether or not they use the same manipulation algorithm.
%!Specifically, proactive defense in the case of ${\sf F}_D={\sf F}_A$
%!is more effective than in the case of ${\sf F}_D\neq {\sf F}_A$.
This phenomenon also can be explained by that the features that are often manipulated by ${\sf F}_1$
are very different from the features that are often manipulated by ${\sf F}_2$.
More specifically, when ${\sf F}_A={\sf F}_D$, the proactively learned classifiers $M_1^\dag,\ldots,M_\gamma^\dag$
would capture the ``maliciousness" information embedded in the manipulated data $D_\alpha$;
this would not be true when ${\sf F}_A\neq {\sf F}_D$.
Moreover, the ${\tt sequential}$ adaptation strategy appears to be more ``oblivious" than the other two strategies
in the sense that $D_\alpha$ preserves less information about $D_0$.
%!This may explain why the false-negative rates when ${\sf ST}_A={\sf ST}_D={\tt sequential}$ can be respectively substantially higher
%!than their counterparts when  ${\sf ST}_A={\sf ST}_D\neq{\tt sequential}$.
%!!The above discussions suggest the following:
%It is important to know the attacker's adaptation strategy ${\sf ST}_A$ and manipulation algorithm ${\sf F}_A$.
%!!{\bf If the attacker is using ${\sf ST}_A={\tt sequential}$,
%!!the defender should not use ${\sf ST}_D={\tt sequential}$}.
% because of the very high false-negative rate,
%whether ${\sf F}_D={\sf F}_A$ or not.}
%It is an interesting future work to identify the optimal manipulation algorithm, if exist.
%!!Third,
%given that the defender should not use ${\sf ST}_D={\tt sequential}$ to counter against ${\sf ST}_A={\tt sequential}$,
what adaptation strategy should the defender use to counter  ${\sf ST}_A={\tt sequential}$?
%!!Table \ref{table:better-strategies} shows that the defender should use ${\sf ST}_D={\tt full}$ because it
%, under the condition ${\sf F}_D={\sf F}_A$,
%!!leads to relatively high detection accuracy. %!and relatively low false-negative rate, while the false-positive rate is comparable to the other cases.
%!!Even if the attacker knows that the defender is using ${\sf ST}_D={\tt full}$,
Table \ref{table:better-strategies} shows that the attacker does not have an obviously more effective counter ${\tt full}$ adaptation strategy.
%Moreover, even if the defender knows that the attacker is using  ${\sf ST}_A={\tt Full}$ adaptation strategy,
% Table \ref{table:better-strategies} shows that the defender does not have an obviously more effective counter adaptation strategy than ${\sf ST}_D={\tt Full}$.
This hints that the ${\tt full}$ strategy may be a kind of equilibrium strategy because
both attacker and defender have no significant gains by deviating from it. This inspires an important problem for future research:
%, with the caveat that more investigations are needed because
%these observations are obtained under the condition  ${\sf F}_D={\sf F}_A$. This leads to:
{\bf Is the ${\tt full}$ adaptation strategy (or variant of it) an equilibrium strategy?}

Third, Table \ref{table:cross-and-aggregation} shows that when ${\sf ST}_D={\sf ST}_A$, the attacker can benefit by increasing
its adaptiveness $\alpha$. %!(i.e., increasing $\alpha$). 
Table \ref{table:better-strategies} exhibits the same phenomenon when ${\sf ST}_D\neq {\sf ST}_A$.
%!On the other hand, by comparing Tables \ref{table:cross-and-aggregation}-\ref{table:better-strategies} and Table \ref{table:attack-power},
%!it is clear that proactive detection $M_{0\text{-}\gamma}(D_\alpha)$ for $\gamma>0$ is much more effective than non-proactive detection $M_0(D_\alpha)$ for $\gamma=0$.
In order to see the impact of defender's proactiveness as reflected by $\gamma$
against the defender's adaptiveness as reflected by $\alpha$,
we plot in Figure \ref{fig:gamma-alpha-f1-f2} how the detection accuracy with respect to $(\gamma-\alpha)$
under the condition ${\sf F}_D={\sf F}_A$ and under various ${\sf ST}_D\times {\sf ST}_A$ combinations.
We observe that roughly speaking, as $\gamma$ increases to exceed
the attacker's adaptiveness $\alpha$ (i.e., $\gamma$ changes from $\gamma<\alpha$ to $\gamma=\alpha$ to $\gamma>\alpha$),
the detection accuracy may have a significant increase at $\gamma-\alpha=0$.
Moreover, we observe that when ${\sf ST}_D={\tt full}$, $\gamma-\alpha$ has no significant impact on the detection accuracy.
This suggest that {\bf the defender should always use the ${\tt full}$ adaptation strategy to alleviate
the uncertainty about the attacker's adaptiveness $\alpha$}.

